Modeling Tiered Pricing in the Internet Transit Market

ISPs are increasingly selling "tiered" contracts, which offer Internet connectivity to wholesale customers in bundles, at rates based on the cost of the links that the traffic in the bundle is traversing. Although providers have already begun to implement and deploy tiered pricing contracts, little is known about how such pricing affects ISPs and their customers. While contracts that sell connectivity on finer granularities improve market efficiency, they are also more costly for ISPs to implement and more difficult for customers to understand. In this work we present two contributions: (1) we develop a novel way of mapping traffic and topology data to a demand and cost model; and (2) we fit this model on three large real-world networks: an European transit ISP, a content distribution network, and an academic research network, and run counterfactuals to evaluate the effects of different pricing strategies on both the ISP profit and the consumer surplus. We highlight three core findings. First, ISPs gain most of the profits with only three or four pricing tiers and likely have little incentive to increase granularity of pricing even further. Second, we show that consumer surplus follows closely, if not precisely, the increases in ISP profit with more pricing tiers. Finally, the common ISP practice of structuring tiered contracts according to the cost of carrying the traffic flows (e.g., offering a discount for traffic that is local) can be suboptimal and that dividing contracts based on both traffic demand and the cost of carrying it into only three or four tiers yields near-optimal profit for the ISP.

==> ack.tex <==
\section*{Acknowledgments}

We are grateful to the anonymous reviewers and our shepherd, David Clark,
for feedback.
%
We thank Guavus for early feedback and help with data.
%
This research was primarily supported by grant N000140910755 from the
Office of Naval Research.  Vytautas Valancius and Nick Feamster were also
supported by NSF CAREER Award CNS-06943974.
%
Cristian Lumezanu was supported by NSF Grant 0937060 to the Computing
Research Association for the CIFellows Project.
%
Ramesh Johari was supported in part by NSF grants CMMI-0948434,
CNS-0904609, CCF-0832820, and CNS-0644114.
%
Vijay Vazirani was supported by NSF grants CCF-0728640 and CCF-0914732,
and a Google Research Grant.  


==> arxiv.tex <==
\begin{abstract}

ISPs are increasingly selling ``tiered'' contracts, which offer Internet
connectivity to wholesale customers in bundles, at rates based on the
cost of the links that the traffic in the bundle is traversing. Although
providers have already begun to implement and deploy tiered pricing
contracts, little is known about how such pricing affects ISPs and their
customers. While contracts that sell connectivity on finer granularities
improve market efficiency, they are also more costly for ISPs to
implement and more difficult for customers to understand.  In this work
we present two contributions: (1)~we develop a novel way of mapping
traffic and topology data to a demand and cost model; and (2)~we fit this
model on three large real-world networks: an European transit ISP, a
content distribution network, and an academic research network, and run
counterfactuals to evaluate the effects of different pricing strategies
on both the ISP profit and the consumer surplus. We highlight three core
findings. First, ISPs gain most of the profits with {\em only three or
four pricing tiers} and likely have little incentive to increase
granularity of pricing even further. Second, we show that {\em consumer
surplus follows closely, if not precisely, the increases in ISP profit}
with more pricing tiers. Finally, the common ISP practice of structuring
tiered contracts according to the cost of carrying the traffic flows
(\eg{}, offering a discount for traffic that is local) can be suboptimal
and that dividing contracts based on {\em both traffic demand and the
cost of carrying it} into {\em only three or four tiers} yields
near-optimal profit for the ISP.


\end{abstract}
\section*{Acknowledgments}

We are grateful to the anonymous reviewers and our shepherd, David Clark,
for feedback.
We thank Guavus for early feedback and help with data.
This research was primarily supported by grant N000140910755 from the
Office of Naval Research.  Vytautas Valancius and Nick Feamster were also
supported by NSF CAREER Award CNS-06943974.
Cristian Lumezanu was supported by NSF Grant 0937060 to the Computing
Research Association for the CIFellows Project.
Ramesh Johari was supported in part by NSF grants CMMI-0948434,
CNS-0904609, CCF-0832820, and CNS-0644114.
Vijay Vazirani was supported by NSF grants CCF-0728640 and CCF-0914732,
and a Google Research Grant.  
\section{Background}
\label{sec:background}

In this section, we describe the current state of affairs in the Internet transit
market. We first taxonomize {\em what} services (bundles) ISPs are
selling. We then provide intuition on {\em why} ISPs are moving towards
tiered wholesale Internet transit service.

\subsection{Current Transit Market Offerings}
\label{sec:services}

Unfortunately, there is not much public information about the wholesale
Internet transit market. ISPs are reluctant to reveal specifics about
their business models and pricing strategies to their competitors.
Therefore, to obtain most of the information in this section, we engaged in
many discussions and email exchanges with network operators.  Below, we
classify the types of Internet transit service we identified during
these conversations.  Although much of the information in this section is
widely known in the network operations community, it is difficult to find
a concise taxonomy of product offerings in the wholesale transit market.
The taxonomy below serves as a point of reference for our discussions of
tiered pricing in this paper, but it may also be useful for anyone who
wishes to better understand the state of the art in pricing strategies in
the wholesale transit market.

\para{Peering} business relationships (or, more formally, {\em
settlement-free peering} relationships) have been extensively studied by
networking researchers~\cite{Johari2003, Chang:infocom2006,
Dhamdhere2010, Feamster2004b, Feamster2004c} and well-documented in the
industry white papers~\cite{Norton-www}. Most peering connections are
established through public Internet eXchange Points (IXP), while higher
bandwidth peering often requires private peering sessions. A network
engaging in a settlement free peering allows its peer to reach {\em
on-net} destinations---destinations in its own network, and destinations
in customer networks. For the peering to be settlement-free, most ISPs
pose a set of requirements to prospective peers, such as number of
interconnection points, geographic coverage, or ingress/egress traffic
ratios. If an ISP cannot meet peering requirements, it is forced to buy
Internet {\em transit} or {\em paid peering}~\cite{l3-cogent-depeering,
telia-cogent-depeering, www-he-cogent-depeering}.

\para{Transit.} Most ISPs offer conventional Internet transit service.
Internet transit is sold at a {\em blended rate}---a single price
(usually expressed in \$/Mbps/month)---charged for traffic to all
destinations. Historically, blended rates have been decreasing by 30\%
each year~\cite{Norton-www}. Blended rate is the simplest and yet the
most crude way to charge for traffic. If network costs are highly
variable, less costly flows in the blended-rate bundle subsidize other,
more expensive flows. ISPs often innovate by offering more than one rate:
We summarize three pricing models that require two or more rates:
(1)~{\em paid peering}, (2)~{\em backplane peering}, and (3)~{\em
regional pricing}.


\para{Paid peering} is similar to settlement-free peering, except that
one network pays to reach the other. A major ISP might separately sell
{\em off-net} routes (wholesale transit) at one rate and {\em on-net}
routes (to reach destinations inside its own network) at another (usually
lower) rate. For example, national ISPs in Eastern Europe, Australia, and
in other regions may sell local connectivity at a discount to increase
demand for local traffic, which is is significantly cheaper than transit
to outside global destinations~\cite{www-adam-unmetered}.  The on-net
routes are also offered at a discount by some major transit ISPs to large
content providers, because such transit ISPs can recoup part of the costs
from their customers, who congest paid upstream links to transit ISPs by
downloading the content. Some instances of paid peering have spawned
significant controversy: most recently, Comcast---primarily a network
serving end-users---was accused of a network neutrality violation when it
forced one tier-1 provider to pay to reach Comcast's
customers~\cite{www-comcast-vs-level3}.

\para{Backplane peering} occurs when an ISP, in addition to selling
global transit through its own backbone, charges a discount rate for the
traffic it can offload to its peers at the same Internet exchange.
Smaller ISPs buy such a service because they might not meet all the
settlement-free peering requirements to peer directly with the ISPs in
the exchange. Although many large ISPs discourage this practice, some
ISPs deviate by offering backplane peering to retain customers or to
maintain traffic ratios with their peers. As with paid peering, the ISP
selling backplane peering has to account and charge for at least two
traffic flows: one to peers and another to its backbone.

\para{Regional pricing} occurs when transit service providers offer
different rates to reach different geographic regions. The regions can be
defined at different levels of granularity, such as PoP, metro
area, regional area, nation, or continent. In some instances, the
transit ISP offers access to all regions with different prices; in other
instances, the downstream network purchases access only to a specific
geographic region (\eg{}, access only to South America or Australia). In
practice, due to the overhead of provisioning and maintaining many
sessions to the same customer, ISPs rarely use more than one or two extra
price levels for different regions.

We speculate that the bundling strategies described above arose primarily
from operational and cost considerations. For example, it is relatively
easy for a transit ISP to tag which routes are coming from customers and
which routes are coming from peers and then in turn sell them separately
to its customers. Similarly, it is relatively easy to sell local (\ie,
less costly) routes separately. We show that these na\"{i}ve bundling
strategies might not be as effective as bundling strategies that account
for both cost and demand.



\subsection{The Trend Towards Tiered Pricing}
\label{sec:motivation}

Conventional blended rate pricing is simple to implement, but it may be
inefficient.  ISPs can lose profit as a result of blended-rate pricing,
and customers can lose surplus.  This is an example of {\em market
failure}, where goods are not being efficiently allocated between
participants of the market.  Another outcome of blended-rate pricing is
the {\em increase in direct peering} to circumvent ``one-size-fits-all''
transit.  Both phenomena provide incentives for ISPs to improve their
business models to retain revenue.  We now explain each of these
outcomes.


\begin{figure}[t!]
  \centering
  \subfigure[{\bf Blended-rate pricing.} ISP charges a single blended
  rate $P_0$.]{
  \includegraphics[width=0.7\linewidth]{fig/bundled}
  \label{fig:bundled_pricing}}
  \subfigure[{\bf Tiered pricing.} ISP charges rates $P_1$ and $P_2$ for flows.]{
  \includegraphics[width=0.7\linewidth]{fig/unbundled}
  \label{fig:unbundled_pricing}}
  \centering
  \caption{Market efficiency loss due to coarse bundling.}
  \label{fig:inefficiency}
\end{figure}


\subsubsection{Profit and surplus loss} 

Selling transit at a blended rate could reduce profit for transit ISPs
and surplus for customers. We define an ISP's {\em profit} as its revenue
minus its costs, and {\em customer surplus} as customer utility minus the
amount it pays to the ISP. Unrealized profit and surplus can occur when
ISPs charge a single rate while incurring different costs when delivering
traffic to destinations.


Figure~\ref{fig:inefficiency} illustrates how tiered pricing can increase
both the profit for an ISP and the surplus for a customer. The
downward-sloping curves represent consumer demand\footnote{We model
consumer demand as {\em residual demand}. Residual demand  accounts for
consumption change both due to inherent consumer demand and due to some
consumers shifting consumption to substitutes, such as other ISPs (See
Section~\ref{sec:ced}.)} to two destinations.  Since the demand slope
$D_2$ is higher than demand slope $D_1$, the customer has higher
demand for the second destination in the ISP's network. Assume that the
ISP cost of serving demand $D_1$ is \$1, while the cost of serving demand
$D_2$ is \$0.5.  Modeling demand with constant elasticity
(Section~\ref{sec:model}), the {\em profit maximizing price} can be shown
to be $P_0=\$1.2/Mbps$.  If, however, the ISP is able to offer two
bundles, then the profit maximizing prices for such bundles would be
$P_1=\$2.7$ and $P_2=\$1$.  Figure~\ref{fig:unbundled_pricing} shows that
this price setup not only increases ISP profit but also increases
consumer surplus and thus social welfare. 

The market achieves higher efficiency because customers adjust their
consumption levels of the ISP network according to their demand and to
the prices that the ISP exposes, which directly depend on its costs.
Without the ISP's indirect exposure of its costs, the customer consumes
less of the cheaper capacity and more of the expensive capacity than it
would otherwise. In Section~\ref{sec:model}, we formalize the market that
we have used in this example and propose more complex demand and cost
models.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.6\linewidth]{fig/cdn-game}

  \caption{The customer procures a direct link if the
  cost for such a link is lower than the blended rate  $c_{direct} <  R$.}
  
  \label{fig:cdn-game} 
\end{figure}


\subsubsection{Increase in direct peering} 

Charging for traffic at a blended rate also provides incentives for
client networks to connect directly to georgraphically close Internet
Exchange Points (IXPs). For
instance, if a transit ISP charges only blended rate, client network
might find geographically close IXPs cheaper to reach by leasing or
purchasing private links. While direct peering is generally perceived as
a positive phenomenon, for transit ISPs it means less revenue. Direct
peering efforts can also diminish economies of scale: instead of using
shared ISP infrastructure, customers provision their own connectivity to
IXPs. 

Figure~\ref{fig:cdn-game} illustrates an interaction between an upstream
ISP and a CDN client (\eg{}, Google, Microsoft) with its own
backbone, which extends to the NYC PoP. The CDN might, or might not, have
a content cache at the Boston IXP, but since it does not have its own
backbone presence at the IXP, the CDN must pay the upstream ISP to reach
it.  The ISP offers a blended rate $R$ at the the NYC PoP for all the
traffic, including the traffic to the Boston IXP. The blended rate $R$ is
set to compensate the upstream provider for the overall traffic mix and,
therefore, is {\em higher} than the amortized cost of most of the cheaper
(more localized) flows that ISP is serving (\ie{}, the flows between the
NYC and Boston PoPs). The CDN eventually will procure a direct link to
the Boston IXP, if it finds that it can procure such a direct link at an
amortized cost $c_{direct} < R$.  Assuming the ISP's profit margin is $M$
and flow accounting overhead is $A$ (discussed in
Section~\ref{sec:accounting}), such a direct link presents a {\em market
failure} if $c_{direct} > (M+1)c_{ISP} + A$, because the customer deploys
additional capacity at a higher cost than the ISP could have charged in a
tiered market.

Some operators we interviewed confirm that they periodically re-evaluate
transit bills and expand their backbone coverage if they find that having
own presence in an IXP pays off. In today's transit market, many
customers increasingly opt for direct
peering~\cite{Labovitz:sigcomm2010}; transit service providers are
absorbing losses as a result of competitive pressure~\cite{Norton-www}.
Naturally, this pressure increases the incentive for ISPs to adopt a
tiered pricing model for local traffic. The central question, then, is
how they should go about structuring these tiers. The rest of the paper
focuses on this question.
\section{Conclusion}\label{sec:conclusion}


As the price of Internet transit drops, transit providers are selling
connectivity using ``tiered'' contracts based on traffic cost,
volume, or destination to maintain profits. 
We have studied two questions: How does tiered pricing benefit the ISPs?
and How does tiered pricing affect their customers?
We developed a model for an Internet transit market that helps us to
evaluate differing pricing strategies of the ISPs.
We have applied our model to traffic demand and topology data from three
large ISPs to evaluate various bundling strategies.

We find that the ISPs gain most of the profits with {\em only three or
four pricing tiers} and likely have little incentive to icnrease
granularity of pricing even further. We also show that consumer surplus
follows closely, if not precisely, the increases in ISP profit with more
pricing tiers. 
\section{Evaluating Tiered Pricing}
\label{sec:eval}

\begin{figure}
\centering
\includegraphics[width=0.7\linewidth]{fig/transit-model}
\caption{We evaluate the effect of tiered pricing on Internet transit by
separately modeling the demand and cost of traffic. At each step we use real-world data to derive
unknown parameters.}
\label{fig:transit-model}
\end{figure}


In this section, we evaluate the efficiency of destination-based tiered
pricing using the model presented in Section~\ref{sec:model} and real
topology and demand data from large  networks.  Our goal is to understand
how the consumer surplus and the profit that an ISP extracts from
offering tiered-pricing depends on the number of tiers and the network
topology and traffic demand. One of the major challenges we face is that we cannot know some aspects
of the cost and demand models, or even which model to use. We use the ISP
data to derive model parameters, such as valuation or cost, and evaluate
the profit of each strategy across models and input parameters.
Figure~\ref{fig:transit-model} presents an overview of our approach.

Our evaluation yields several important results. First, we show that an
ISP needs only 3--4 bundles to capture 90--95\% of the profit provided by
an infinite number of bundles, if it bundles the traffic appropriately.
Second, choosing a bundling strategy that considers both flow demand and
cost is almost as effective as an exhaustive search for the best
combination of bundles. Finally, we observe that the topology and traffic
of a network influences its bundling strategies: networks with higher
coefficient of variation of demand need more bundles to extract maximum
profit.

\vspace{-3mm}
\subsection{Mapping Data to Models}\label{sec:mapping}
\label{sec:eval1}

Because we do not know the parameters that we need to compute the
profit-maximizing prices we must derive them.  We first describe the data
then we show how to apply the demand models to the real traffic demands
to compute the valuation coefficients $v_i$ for each flow $i$. Finally,
we derive the ISP's cost for servicing the flows by applying cost models
to the observed flow distances.

\begin{table}
\small
\centering
\begin{tabular}{|l||c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Data set}} 	& \multirow{2}{*}{\textbf{Date}} &
\multicolumn{2}{c|}{\textbf{Distance (miles)}} & \multicolumn{2}{c|}{\textbf{Traffic (Gbps)}}\\
\cline{3-6} &  & \textbf{w-avg} & \textbf{CV} & \textbf{Aggregate} & \textbf{CV}\\
\hline
EU ISP			& 11/12/09     & 54 & 0.70 & 37 & 1.71 \\
CDN			& 12/02/09     & 1988 & 0.59 & 96 & 2.28  \\
Internet 2		& 12/02/09     & 660 & 0.54 & 4 & 4.53 \\
\hline
\end{tabular}
\caption{Data sets used in our evaluation. The columns represent: the
network, data capture date, demand-weighted average of flow distances,
coefficient of variation (CV) of flow distances, aggregate traffic per
second, and CV of demand of different flows.}
\label{tab:datasets}
\end{table}


\subsubsection{Data Sources}
\label{sec:data}

We use demand and topology data from three networks: a European ISP
serving thousands of business customers (EU ISP), one of the largest CDN
providers in the world (CDN), and a major research network in United
States (Internet 2). The data consists of sampled NetFlow records from
core routers in each network for 24 hours.  Table~\ref{tab:datasets}
presents more details about the data sets.

To drive our model, we must compute the traffic volume (which captures
consumer demand) and the distance between the source and destination of
each flow (which captures the relative cost of transit).  To do so, we
extract the source and destination IP, as well as the traffic level, from
each NetFlow record. We obtain the demand for each flow by aggregating
all records of the flow, while ensuring that we do not double-count
record duplicated on different routers.

To compute distances that reflect the ISP's cost of sending traffic, we
use the following heuristics. For the EU ISP, the distance that each flow
travels in the ISP's network is the geographical distance between the
flow's entry and exit points, whose identity and location is known. For
the CDN, we use the GeoIP database~\cite{www-geoip} to estimate the
distance to the destination. Although this may not reflect the real
distance that a packet travels (because part of the path may be covered
by another ISP), we assume that it is still reflective of the cost
incurred by the CDN.  Finally, for Internet2 we use the router interface
information to identify the links the flow has traversed. The distance
each flow traverses is the sum of the links in the path, where the link
length is the geographical distance between the neighboring routers.

\subsubsection{Discovering valuation coefficients}

The valuation coefficient $v_i$ indicates the valuation of flow $i$. We
need the valuation coefficeint $v_i$ to capture how the demand for flow
$i$ varies with price (Equations~\ref{eqn:demand-ced}
and~\ref{eqn:demand-logit}) and thus affect the ISP profit. To find $v_i$
for each flow, we assume that ISPs charge the same blended price $P_0$
for each flow and map the observed traffic demand from the data to each
demand model. 

\para{CED valuation coefficient.} From Equation~\ref{eqn:demand-ced} we
obtain:

\vspace{-2mm}
\begin{equation}
  \textstyle v_i = P_0q_i^{1/\alpha},
\end{equation}

\noindent where $q_i$ is observed demand on flow $i$ and $\alpha$ is the
sensitivity coefficient that we vary in the evaluation.

\para{Logit demand valuation coefficient.} Dividing both left and right
sides of market share expression (Equation~(\ref{eqn:marketshare}) by the
corresponding sides of $s_0$ (Equation~(\ref{eqn:share-zero})), we can
find valuation of flow $i$:

\vspace{-2mm}
\begin{equation}
  \textstyle v_i = \frac{\log s_i - \log s_0}{\alpha} + P_0,
\end{equation}

\noindent where $s_i$ is the market share of flow $i$. We vary $s_0$ in the
evaluation and compute the remaining market shares from observed traffic
as $s_i = \frac{q_i(1-s_0)}{\sum q_i}$.

\subsubsection{Discovering costs}
\label{sec:reconsile}

To estimate the ISP profit, we must know the cost that an ISP incurs to
service each flow. However, the data provides information only about the
distance each flow traverses, which reflects only the relative cost
(\eg{}, flow A is twice as costly as flow B), rather than an absolute
cost value. To normalize the cost of carrying traffic to the same units
as the price for the flow, we introduce a scaling parameter $\gamma$,
where $c_i = \gamma f(d_i)$ and $d_i$ is the distance covered by $i$ (see
Section~\ref{sec:cost-model}). For each demand model, we compute the
scaling parameter by assuming (as in computing valuation coefficients)
that ISPs are rational and profit maximizing, and charge the same
original price $P_0$ for each flow.

\para{CED.} Differentiating profit Equation~(\ref{eqn:profit-ced}) in
terms of price and then substituting $c_i$ with $\gamma f(d_i)$, we find
cost normalization coefficient:

\vspace{-3mm}
\begin{equation}
  \gamma = \frac{P_0(\alpha-1)\sum_{i=1}^n v_i^\alpha}{\alpha\sum_{i=1}^n
  f(d_i)v_i^\alpha}
\end{equation}

\para{Logit demand.} Like in CED case, differentiating profit
Equation~\ref{eqn:logit-profit} and substituting $c_i$ for $\gamma
f(d_i)$, we can express $\gamma$:

\vspace{-3mm}
\begin{equation}
  \gamma = \frac{\sum_{i=1}^n\left(e^{\alpha(v_i-P_0)}\left(\alpha P_0 - 1
  - \sum_{j=1}^n e^{\alpha(v_j-P_0)}\right)\right)}{\alpha \sum_{i=1}^n
  f(d_i)e^{\alpha(v_i-P_0)} }
\end{equation}

\vspace{-3mm}

\subsection{Effects of Tiered Pricing}
\label{sec:bundling}

ISPs must judiciously choose how they bundle traffic flows into tiers. As
shown in Section~\ref{sec:services}, today's ISPs often offer at most two
or three bundles with different prices. We define six bundling strategies
that classify and group traffic flows according to their cost, demand, or
potential profit to the ISP. We then evaluate them and show that,
assuming the right bundling strategy is used, ISPs typically need only a
few bundles to collect near-optimal profit.

\begin{figure*}
  \subfigure[European
  ISP.]{\includegraphics[width=0.33\linewidth]{fig/vm-ced-bundling}}
  \subfigure[Internet2.]{\includegraphics[width=0.33\linewidth]{fig/i2-ced-bundling}}
  \subfigure[International
  CDN.]{\includegraphics[width=0.33\linewidth]{fig/ll-ced-bundling}}
  \caption{Profit capture for different bundling strategies in constant
  elasticity demand.}
  \label{fig:ced-division-types}
\end{figure*}

\begin{figure*}
  \subfigure[European ISP.]{\includegraphics[width=0.33\linewidth]{fig/vm-logit-intervals}}
  \subfigure[Internet2.]{\includegraphics[width=0.33\linewidth]{fig/i2-logit-intervals}}
  \subfigure[International CDN.]{\includegraphics[width=0.33\linewidth]{fig/ll-logit-intervals}}
  \caption{Profit capture for different bundling strategies in logit demand.}
  \label{fig:logit-division-types}
\end{figure*}

\subsubsection{Bundling strategies}
\label{sec:bundling-strategies}

\para{Optimal.} We exhaustively search all possible combinations of
bundles to find the one that yields the most profit. This approach gives
optimal results and also serves as our {\em baseline} against which we
compare other strategies. Computing the optimal bundling is
computationally expensive: for example, there is more than a billion ways
to divide one hundred traffic flows into six pricing bundles. Presented
below, all of the other bundling strategies employ heuristics to make
bundling computationally tractable.

\para{Demand-weighted.} In this strategy, we use an algorithm inspired
by token buckets to group traffic flows to bundles. First, we set the
overall token budget as the sum of the original demand of all flows:
$T=\sum_i q_i$. Then, for each bundle $j$ we assign the same token
budget $t_j=T/B$, where $B$ is the number of bundles we want to create.
We sort the flows in decreasing order of their demand and traverse them
one-by-one. When traversing flow $i$, we assign it to the first bundle
$j$ that either has no flows assigned to it or has a budget $t_j>0$. We
reduce the budget of that bundle by $q_i$. If the resulting budget
$t_j<0$, we set $t_{j+1}=t_{j+1} + t_j$. After traversing all the flows,
the token budget of every bundle will be zero, and each flow will be
assigned to a bundle. The algorithm leads to separate bundles for high
demand flows and shared bundles for low demand flows. For example, if we
need to divide four flows with demands 30, 10, 10, and 10 into two
bundles, the algorithm will place the first flow in the first bundle,
and the other three flows in the second bundle.

\para{Cost-weighted.} We use the same approach as in demand-weighted
bundling, but we set the token budget to $T=\sum_i 1/c_i$. When placing
a flow in a bundle we remove a number of tokens equal to the inverse of
its cost.  This approach creates separate bundles for local flows and
shared bundles for flows traversing longer distances. The current ISP
practices of offering {\em regional pricing} and {\em backplane peering}
maps closely to using just two or three bundles arranged using this
cost-weighted strategy.

\para{Profit-weighted.} The bundling algorithms described above consider
cost and demand separately. To account for cost and demand together, we
estimate {\em potential profit} each flow could bring. We use the
potential profit metric to apply the same weighting algorithm as in cost
and demand-weighted bundling. In case of constant elasticity demand, we
derive potential profit of each flow $i$:

\vspace{-4mm}
\begin{equation}
  \pi_i = \frac{v_i^\alpha}{\alpha}
  \left(\frac{\alpha c_i}{\alpha-1}\right)^{1-\alpha}
\end{equation}

For the logit demand, substituting $p_i$ in
Equation~\ref{eqn:logitprofit} yields:

\begin{equation}
  \pi_i = Ks_i(p_i-c_i) = \frac{Ks_i}{\alpha s_0}\propto q_i
\end{equation}


\para{Cost division.} We find the most expensive flow and divide
the cost into ranges according to that value.  For example, if we want to
introduce two bundles and the most expensive flow costs
\$10/Mbps/month to reach, we assign flows that cost \$0--\$4.99 to the
first bundle and flows that cost \$5--\$10 to the second bundle.

\para{Index division.} Index-division bundling is similar to cost
division bundling, except that we rank flows according to their cost and
use the rank, rather than the cost, to perform the division into
bundles.

\subsubsection{The effects of different bundling strategies}
\label{sec:effects1}

To evaluate the bundling strategies described above, we compute the
profit-maximizing prices and measure the resulting pricing outcome in
terms of {\em profit capture}. Profit capture indicates what fraction of
the maximum possible profit---the profit attained using an infinite
number of bundles---the strategy captures. For example, if the maximum
attainable profit is 30\% higher than the original profit, while the
profit from using two bundles is 15\% higher than the original profit,
the profit capture with two bundles attains 0.5 of profit capture.
Formally, profit capture is $(\pi_{\mathsf{new}} -
\pi_{\mathsf{original}})/(\pi_{\mathsf{max}}-\pi_{\mathsf{original}})$.

Figures~\ref{fig:ced-division-types} and~\ref{fig:logit-division-types}
show the profit capture for different bundling strategies, across the
three data sets, while varying the number of bundles. For the results
shown here, we use both the constant elasticity and the logit demand
models and the linear cost model. We set the price sensitivity $\alpha$
to $1.1$, the original, blended rate $P_0$ to $\$20$, the cost tuning
parameter $\theta$ to $0.2$, and the original market fraction that sends no
traffic $s_0$ to $0.2$.  We explore the effect of varying these
parameters in Section~\ref{sec:sensitivity}. 


\para{Optimal versus heuristics-based bundling.} With an appropriate
bundling strategy, the ISP attains maximum profit with just 3--4
bundles.  As expected, the optimal flow bundling strategy captures the
most profit for a given number of bundles. We observe that the EU ISP
captures more profit with two bundles than other networks. We attribute
this effect to the low coefficient of variation (CV) of demand to
different destinations, which limits the benefits of having more pricing
bundles. We also discover that, given fixed demand, a high CV of
distance (cost) leads to higher absolute profits. With only minor exceptions,
the profit-weighted bundling heuristic is almost as good as the the
optimal bundling, followed by the cost-weighted bundling
heuristic. Deeper analysis, beyond the scope of this work, could show
what specific input data conditions cause the profit-weighted flow
bundling heuristic to produce bundlings superior to the cost-weighted
heuristic.

\para{Logit profit capture.} Maximum profit capture occurs more quickly
in the logit model because (1)~the total demand (including $s_0$ option)
is constant, and (2)~the model is sensitive to differences in
valuation of different flows. When there is a flow with a significantly
higher difference between valuation and cost ($v_i-c_i$), it absorbs most
of the demand. In this model, with just two pricing tiers, local and
non-local traffic are separated into distinct bundles that closely
represent the {\em backplane peering} and {\em regional pricing} for
local area service models.

\begin{figure}[h!]
  \centering
  \subfigure[Constant elasticity
  demand.]{\includegraphics[width=0.7\linewidth]{fig/ced-capture}}
  \subfigure[Logit.]{\includegraphics[width=0.7\linewidth]{fig/logit-capture}}
  \caption{ISP profit and consumer surplus change as ISP employ an
  increasing number of pricing tiers. Concave cost model, $\theta=0.2$,
  $\alpha=1.1$, $s_0=0.2$.}
  \label{fig:profit-capture}
\end{figure}


\subsubsection{Pricing effects on consumer surplus}

Figure~\ref{fig:profit-capture} contrasts consumer surplus change next to
ISP profit gains. The consumer surplus here is normalized to the surplus
gain the consumers get when ISPs maximize their profit with an infinite
number of pricing tiers. As expected, the surplus gain follows closely,
if not precisely, ISP profit gains.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/vm-linear}
  \caption{Profit increase in EU ISP network using linear cost model.}
  \label{fig:linear-cost}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/vm-concave}
  \caption{Profit increase in EU ISP network using concave cost model.}
  \label{fig:concave-cost}
\end{figure}


\subsection{Sensitivity Analysis}
\label{sec:sensitivity}

We explore the robustness of our results to cost models and input
parameter settings. As we vary an input parameter under test, other
parameters remain constant. Unless otherwise noted, we use
profit-weighted bundling, the EU ISP dataset, sensitivity $\alpha=1.1$,
the linear cost model with base cost $\theta=0.2$, blended rate
$P_0=\$20.0$, and, in the logit model, $s_0=0.2$ (the original market
fraction that sends no traffic).

\subsubsection{Effects of cost models}
\label{sec:cost-eval}

We aim to see how cost models and settings within these models
qualitatively affect our results from the previous section. We show how
profit changes as we increase the number of bundles for different
settings of the cost model parameters ($\theta$), described in
Section~\ref{sec:cost-model}. We find that for different $\theta$
settings most of the attainable profit is still captured in 2-3 bundles.
Unlike in other sections, in
Figures~\ref{fig:linear-cost}--\ref{fig:type-cost},
we normalize the profit of all the plots in the
graphs to the highest observed profit. In other words, $\pi_{max}$ in
these figures is not the maximum profit of each plot, but the maximum
profit of the plot with highest profit in the figure. Normalizing
by the highest observed profit allows us to show how changing
the parameter $\theta$ affects the amount of profit that the ISP can
capture.

\para{Linear cost.} 
Figure~\ref{fig:linear-cost} shows profit increase in the EU ISP network
as we vary the number of bundles for different settings of $\theta$. As
expected, most of the profit is still attained with 2--3 pricing bundles.
We also observe that the increase in the base cost ($\theta$) causes
a decline in the maximum attainable profit. The reduction in maximum
attainable profit is expected, as increasing the base cost reduces the
coefficient of variation (CV) of the cost of different flows and thus reduces
the opportunities for variable pricing and profit capture. We can also
see, as shown in previous section, that the logit demand model attains
more profit than the constant elasticity demand model with the same
number of pricing bundles.

\para{Concave cost.} Figure~\ref{fig:concave-cost} shows the profit
increase as we vary the number of bundles for different
settings of $\theta$ for the concave cost model. The observations and results
are similar to the linear cost model, with one notable exception. The amount
of profit the ISP can capture decreases more quickly in the concave cost model than in
the linear cost model for the same change in the base-cost parameter $\theta$.
This is due to the lower CV of cost in the concave model than in the linear cost
model. In other words, applying the log function on distance (as described in
Section~\ref{sec:cost-model}) reduces the relative cost difference between
flows traveling to local and remote destinations. 

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/vm-region}
  \caption{Profit increase in the EU ISP network using  regional cost model.}
  \label{fig:regional-cost}
\end{figure}

\para{Regional cost.} In the regional cost model, the parameter $\theta$ is
an exponent which adjusts the price difference between three different
regions: local, national, and international.
Figure~\ref{fig:regional-cost} shows the profit increase in the EU ISP
network as we vary number of bundles for different settings of $\theta$.
Higher $\theta$ values result in a higher CV of cost in different
regions which, in turn, in both demand models produces higher profit.
Using constant elasticity demand we observe a small dip in profit when
using five and six bundles, which recovers later with more bundles. Such
dips are expected when there are only a few traffic classes. For example, if traffic
had just two distinct cost classes, two judiciously selected bundles
could capture most of the profit. Adding a third bundle can reduce the
profit if that third bundle contains flows from both of the classes
(as may happen in a suboptimal bundling).

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/vm-type}
  \caption{Profit increase in the EU ISP network using destination type cost model.}
  \label{fig:type-cost}
\end{figure}

\para{Destination type-based cost.} Destination type-based cost model
emulates ``on-net'' and ``off-net'' types of traffic in an ISP network.
As described in Section~\ref{sec:cost-model}, we assume that ``on-net''
traffic costs less than ``off-net'' traffic. We vary $\theta$, which
represents a fraction of ``on-net'' traffic in each flow. The standard
profit-weighting algorithm does not work well with the destination
type-based cost model. The effect observed in the regional cost
model---where five bundles produce slightly lower profit then four
bundles---is 
more pronounced when we have just two distinct flow classes. One
heuristic that works reasonably well is as follows: we update the
profit-weighting heuristic to never group traffic from two different
classes into the same bundle.  Figure~\ref{fig:type-cost} shows how
profit increases with an increasing number of bundles. Since there are
two major classes of traffic (``on-'' and ``off-net''), most profit is
attained with two bundles for both demand models. In this cost model, as
in other cost models, the same change in CV of cost (induced by the
parameter $\theta$) causes a greater change in profit capture for
constant elasticity demand than for logit demand.



\subsubsection{Sensitivity to parameter settings}

The models we use rely on a set of parameters, such as price sensitivity
($\alpha$), price of the original bundle ($P_0$), and, in the logit
model, the share of the market that corresponds to deciding not to
purchase bandwidth ($s_0$). In this section, we analyze how sensitive
the model is to the choice of these parameters.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/alpha-sensitivity}
  \caption{Minimum profit capture for a fixed number of bundles over a range of $\alpha$ between 1 and
  10.}
  \label{fig:alpha-sensitivity}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/pzero-sensitivity}
  \caption{Minimum profit capture for a fixed number of bundles over a range of
  starting prices $P_0\in[5,30]$.}
  \label{fig:pzero-sensitivity}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/szero-sensitivity}
  \caption{Maximum profit capture for a fixed number of bundles over a range 
  of fractions of users who decide not to participate in the market
  $s_0\in(0,1)$.}
  \label{fig:szero-sensitivity}
\end{figure}

Figures~\ref{fig:alpha-sensitivity}--\ref{fig:szero-sensitivity}
show how profit capture is affected by
varying price sensitivity $\alpha$, blended rate $P_0$, and non-buying
market share $s_0$, respectively.  Each data point in the figures is
obtained by varying each parameter over a range of values.  We vary
$\alpha$ between 1 and 10, $P_0$ between 5 and 30, and $s_0$ between 0
and 0.9. As we vary the parameters, we select and plot the {\em minimum}
observed profit capture over the whole parameter range, for the
profit-weighted strategy with different numbers of bundles. In other
words, these plots show the worst case relative profit capture for the
ISP over a range of parameter values.
The trend of these minimum profit
capture points is qualitatively similar to patterns in
Figures~\ref{fig:ced-division-types} and~\ref{fig:logit-division-types}.
For example, using the CED model and grouping flows in two bundles in the EU
ISP yields around 0.8 profit capture, regardless of price sensitivity,
blending rate, and market share. These results indicate that
our model is robust to a wide range of parameter values.
\section{Implementing Tiered Pricing}
\label{sec:implementation}

ISPs can implement
the type of tiered pricing that we describe in Section~\ref{sec:eval}
without any changes to their existing protocols or infrastructure, and
ISPs may already be using the techniques we describe below.  If that is
the case, they could simply apply a profit-weighted bundling strategy to
re-factor their pricing to improve their profit, possibly without even
making many changes to the network configuration. We describe two tasks
associated with tiered pricing: associating flows with tiers and
accounting for the amount of traffic the customer sends in each tier.


